Communicating Natural Programs to Humans and Machines

The Abstraction and Reasoning Corpus (ARC) is a set of procedural tasks that tests an agent's ability to flexibly solve novel problems. While most ARC tasks are easy for humans, they are challenging for state-of-the-art AI. What makes building intelligent systems that can generalize to novel situations such as ARC difficult? We posit that the answer might be found by studying the difference of \emph{language}: While humans readily generate and interpret instructions in a general language, computer systems are shackled to a narrow domain-specific language that they can precisely execute. We present LARC, the \textit{Language-complete ARC}: a collection of natural language descriptions by a group of human participants who instruct each other on how to solve ARC tasks using language alone, which contains successful instructions for 88\% of the ARC tasks. We analyze the collected instructions as `natural programs', finding that while they resemble computer programs, they are distinct in two ways: First, they contain a wide range of primitives; Second, they frequently leverage communicative strategies beyond directly executable codes. We demonstrate that these two distinctions prevent current program synthesis techniques from leveraging LARC to its full potential, and give concrete suggestions on how to build the next-generation program synthesizers.

==> sec_discussion.tex <==
\section{Conclusion}
We propose \textbf{natural programs} -- instructions that can be interpreted by humans to produce a verifiable output -- as a pathway to building intelligent systems that can solve general tasks given in a natural way. To this end, we present the \emph{Language-complete Abstraction and Reasoning Corpus} (LARC). 
By being simultaneously \emph{DSL-open} and \emph{language-complete}, LARC highlights the distinctive gap between communication to humans and machines: Where programmers struggle to build a program synthesizer, end-users readily communicate the same tasks using words alone. 
We hope that by studying and curating the LARC dataset multiple communities -- such as psychology, cognitive science, and machine learning -- can work together to close this gap.





% From Theo:

% how much harder arc is to the scone dataset. one is scone has a DSL and they break down every program into 5 steps, and have have turkers describe each step individually. an utterance for each step is a clean mapping from which part of the program to which step. in distant supervision, it is not so distant, so you decode the list of 5 step utterances one after another. ARC is a lot harder we do not have a step-wise annotation for each step. It is more natural and fluid, instead of being broken up. We also have fewer labeled tasks (10 percent as much as scone). our DSL is 103 primitives and scone is. no more than 10.

% we can say we are the first to formally studying what will happen if we attempt program synthesis on a DSL-open domain, first ever actually.

% We need to explain why we solve so few tasks in the main paper discussion. 


